Cache peering in multi-tenant 5G networks

Building on the adoption of the Network Functions Virtualization (NFV) and Software Defined Networking (SDN) paradigms, 5G networks promise distinctive features includ- ing the capability to support multi-tenancy. Virtual network operators (VNOs) are expected to co-exist over the shared infrastructure, realizing their network functionality on top of virtualized resources. In this context, we observe the emerging opportunity for establishing synergies between co-located tenants of the infrastructure, in the form of cache peering relationships between co-located VNOs. Upon a cache miss, co-located caches benefit from content cached at their peers, taking advantage of the shared nature of the infrastructure in reducing latencies and traffic overheads. Our approach allows VNOs to autonomously manage their peering links without the involvement of the infrastructure operator.

==> challenges.tex <==
\subsection{Challenges}
